Solving graph compression via optimal transport

We propose a new approach to graph compression by appeal to optimal transport. The transport problem is seeded with prior information about node importance, attributes, and edges in the graph. The transport formulation can be setup for either directed or undirected graphs, and its dual characterization is cast in terms of distributions over the nodes. The compression pertains to the support of node distributions and makes the problem challenging to solve directly. To this end, we introduce Boolean relaxations and specify conditions under which these relaxations are exact. The relaxations admit algorithms with provably fast convergence. Moreover, we provide an exact $O(d \log d)$ algorithm for the subproblem of projecting a $d$-dimensional vector to transformed simplex constraints. Our method outperforms state-of-the-art compression methods on graph classification.

==> Tabular_form_latex_results0.5.tex <==
egin{table*}[t!]  \caption{{f Description of graph datasets, and comparison of accuracy on test data.}  We provide the statistics on the number of graphs, number of classes, average number of nodes, and average number of edges in each dataset. The average classification test accuracy for each training fraction in $\{0.2, \ldots, 0.8\}$ when each graph was (roughly) compressed to half is also shown: the first number in the parentheses for each fraction is the performance with our algorithm, whereas the second that with the REC algorithm. The algorithm that performs better is indicated with bold in each case. The second row of each dataset shows results with the original uncompressed data. 
  \label{tab:compare}}   
  skip 0.1in 
  ddtolength{	abcolsep}{-4.5pt} 
 \centering  
 %egin{center} 
 \small 
  egin{tabular} {*{12}{c}} %{p{0.32in}ddddddddddd} 
  Dataset & method & acc@0.2 & acc@0.3 & acc@0.4 & acc@0.5 & acc@0.6 & acc@0.7 & acc@0.8 
  \hline  	oprule
REC & MSRC_9 & .74$\pm$.01 & .78$\pm$.01 & .82$\pm$.01 & .82$\pm$.01 & .84$\pm$.02 & .83$\pm$.02 & .84$\pm$.01\\
\hline
Heavy &  & .65$\pm$.02 & .71$\pm$.02 & .77$\pm$.01 & .77$\pm$.01 & .79$\pm$.01 & .80$\pm$.01 & .81$\pm$.01\\
\hline
Affinity &  & .67$\pm$.02 & .72$\pm$.00 & .76$\pm$.01 & .77$\pm$.01 & .79$\pm$.03 & .79$\pm$.02 & .80$\pm$.02\\
\hline
Alg. Dist. &  & .67$\pm$.05 & .72$\pm$.05 & .76$\pm$.03 & .77$\pm$.04 & .80$\pm$.03 & .80$\pm$.03 & .81$\pm$.05\\
\hline
OTC & MSRC_9 & {\bf .78$\pm$.02} & {\bf .82$\pm$.00} & {\bf .84$\pm$.00} & {\bf .85$\pm$.00} & {\bf .85$\pm$.01} & {\bf .86$\pm$.01} & {\bf .87$\pm$.01}\\
\hline
\midrule + 
REC & DHFR & .68$\pm$.01 & .70$\pm$.01 & .72$\pm$.01 & .74$\pm$.01 & .75$\pm$.01 & .76$\pm$.01 & .77$\pm$.01\\
\hline
Heavy &  & .72$\pm$.01 & .75$\pm$.01 & .78$\pm$.01 & .78$\pm$.01 & .78$\pm$.01 & .79$\pm$.01 & .80$\pm$.01\\
\hline
Affinity &  & .72$\pm$.01 & .73$\pm$.01 & .75$\pm$.01 & .76$\pm$.01 & .77$\pm$.02 & .77$\pm$.02 & .78$\pm$.01\\
\hline
Alg. Dist. &  & .74$\pm$.01 & .76$\pm$.01 & .77$\pm$.02 & .79$\pm$.02 & .81$\pm$.02 & .82$\pm$.03 & .81$\pm$.03\\
\hline
OTC & DHFR & {\bf .75$\pm$.01} & {\bf .77$\pm$.01} & {\bf .79$\pm$.01} & {\bf .79$\pm$.00} & {\bf .80$\pm$.01} & {\bf .81$\pm$.01} & {\bf .82$\pm$.01}\\
\hline
\midrule + 
REC & MSRC_21C & .49$\pm$.02 & .54$\pm$.01 & .60$\pm$.01 & .63$\pm$.01 & .64$\pm$.01 & .70$\pm$.01 & .74$\pm$.02\\
\hline
Heavy &  & .41$\pm$.02 & .48$\pm$.02 & .52$\pm$.01 & .54$\pm$.01 & .56$\pm$.01 & .60$\pm$.02 & .65$\pm$.01\\
\hline
Affinity &  & .41$\pm$.02 & .49$\pm$.01 & .52$\pm$.01 & .55$\pm$.01 & .56$\pm$.02 & .61$\pm$.02 & .65$\pm$.02\\
\hline
Alg. Dist. &  & .45$\pm$.04 & .50$\pm$.03 & .52$\pm$.02 & .54$\pm$.03 & .53$\pm$.03 & .59$\pm$.03 & .65$\pm$.04\\
\hline
OTC & MSRC_21C & {\bf .56$\pm$.01} & {\bf .61$\pm$.00} & {\bf .66$\pm$.01} & {\bf .67$\pm$.01} & {\bf .70$\pm$.00} & {\bf .76$\pm$.01} & {\bf .78$\pm$.00}\\
\hline
\midrule + 
REC & BZR_MD & .53$\pm$.01 & .55$\pm$.01 & .56$\pm$.02 & .55$\pm$.02 & .56$\pm$.01 & .57$\pm$.01 & .59$\pm$.02\\
\hline
Heavy &  & .50$\pm$.00 & .55$\pm$.00 & .56$\pm$.00 & .52$\pm$.00 & .55$\pm$.00 & .57$\pm$.00 & .56$\pm$.00\\
\hline
Affinity &  & .51$\pm$.01 & .53$\pm$.01 & .53$\pm$.02 & .53$\pm$.02 & .55$\pm$.02 & .57$\pm$.03 & .56$\pm$.03\\
\hline
Alg. Dist. &  & .50$\pm$.02 & .55$\pm$.03 & .56$\pm$.04 & .52$\pm$.03 & .55$\pm$.03 & .57$\pm$.02 & .56$\pm$.04\\
\hline
OTC & BZR_MD & {\bf .53$\pm$.00} & {\bf .57$\pm$.00} & {\bf .55$\pm$.00} & {\bf .58$\pm$.00} & {\bf .57$\pm$.00} & {\bf .61$\pm$.00} & {\bf .60$\pm$.00}\\
\hline
\midrule + 


==> conclusion.tex <==
\section{Conclusion}
We introduced an optimal transport framework for compressing graphs. Our framework can seamlessly encode prior information about the importance of individual nodes, their labels or attributes, and edges in the graph. 

Our perspective hinges on several technical contributions. We first extended the notion of optimal transport on graphs to accommodate undirected edges. We then provided a dual characterization of the optimal transport distance in terms of distributions over the nodes. We could thus view compression as the problem of minimizing the transport cost from a fixed initial distribution supported on all vertices to an unknown target distribution with smaller support.

We introduced binary selection variables in our compression problem to exert a direct control on sparsity. Thus, we could avoid iterative tuning that is required to match a target support in methods that enforce an $\ell_1$ penalty. The resulting formulation entailed a novel Euclidean projection step on the probability simplex under a diagonal transformation. We provided an efficient algorithm to solve this problem. Our approach also led to a related smooth saddle point problem that could be solved very efficiently by standard algorithms.

Beyond its theoretical foundations, our method demonstrated strong empirical performance on two separate tasks.  Specifically, it outperformed state-of-the-art REC algorithm on standard datasets for graph classification. Moreover, it produced compressed graphs that preserved key structural details in real and synthetic examples. 

==> table.tex <==
\begin{table*}[t!]  \caption{{\bf Description of graph datasets, and comparison of accuracy on test data.}  %We provide the statistics on the number of graphs, number of classes, average number of nodes, and average number of edges in each dataset. The average classification test accuracy for each training fraction in $\{0.2, \ldots, 0.8\}$ when each graph was (roughly) compressed to half is shown for each method.  The algorithm that performs better is indicated with bold in each case. 
  \label{tab:compare}}   
  \vskip 0.1in 
  \addtolength{\tabcolsep}{-4.5pt} 
 \centering  
 %\begin{center} 
 \small 
  \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|} %{*{12}{c}} %{p{0.32in}d|d|ddddddd} 
  \toprule 
   Dataset &  method &  acc@0.2 &  acc@0.3 & acc@0.4 &  acc@0.5 &  acc@0.6 &  acc@0.7 & acc@0.8 \\   \hline 
  \toprule 
 
{\bf MSRC\_9} & REC & .738$\pm$.011 & .782$\pm$.010 & .817$\pm$.009 & .818$\pm$.013 & .835$\pm$.020 & .833$\pm$.018 & .840$\pm$.013\\
\hline
graphs: 221 & Heavy & .648$\pm$.019 & .710$\pm$.024 & .766$\pm$.014 & .773$\pm$.010 & .786$\pm$.009 & .796$\pm$.010 & .813$\pm$.009\\
\hline
classes: 8 & Affinity & .665$\pm$.015 & .722$\pm$.005 & .762$\pm$.010 & .774$\pm$.014 & .789$\pm$.026 & .786$\pm$.019 & .801$\pm$.017\\
\hline
nodes: 40.6 & Alg. Dist. & .666$\pm$.048 & .717$\pm$.051 & .756$\pm$.029 & .771$\pm$.039 & .798$\pm$.032 & .803$\pm$.030 & .809$\pm$.046\\
\hline
edges: 97.9 & OTC & {\bf .781$\pm$.019} & {\bf .821$\pm$.003} & {\bf .836$\pm$.004} & {\bf .852$\pm$.002} & {\bf .851$\pm$.006} & {\bf .861$\pm$.007} & {\bf .874$\pm$.012}\\
\hline
\toprule 
{\bf DHFR} & REC & .681$\pm$.011 & .704$\pm$.014 & .724$\pm$.007 & .738$\pm$.009 & .749$\pm$.008 & .756$\pm$.011 & .771$\pm$.011\\
\hline
graphs: 467 & Heavy & .719$\pm$.010 & .751$\pm$.010 & .776$\pm$.012 & .782$\pm$.008 & .777$\pm$.009 & .786$\pm$.014 & .799$\pm$.013\\
\hline
classes: 2 & Affinity & .717$\pm$.013 & .733$\pm$.011 & .745$\pm$.014 & .761$\pm$.014 & .771$\pm$.019 & .767$\pm$.015 & .785$\pm$.013\\
\hline
nodes: 42.4 & Alg. Dist. & .743$\pm$.011 & .761$\pm$.012 & .768$\pm$.022 & .786$\pm$.019 & .810$\pm$.025 & .817$\pm$.033 & .809$\pm$.030\\
\hline
edges: 44.5 & OTC & {\bf .752$\pm$.005} & {\bf .774$\pm$.006} & {\bf .787$\pm$.008} & {\bf .792$\pm$.004} & {\bf .802$\pm$.012} & {\bf .811$\pm$.008} & {\bf .820$\pm$.012}\\
\hline
\toprule 
{\bf MSRC\_21C} & REC & .485$\pm$.016 & .543$\pm$.010 & .595$\pm$.010 & .625$\pm$.013 & .641$\pm$.008 & .696$\pm$.013 & .738$\pm$.016\\
\hline
graphs: 209 & Heavy & .408$\pm$.016 & .479$\pm$.015 & .516$\pm$.009 & .538$\pm$.009 & .557$\pm$.011 & .602$\pm$.022 & .653$\pm$.011\\
\hline
classes: 20 & Affinity & .413$\pm$.021 & .489$\pm$.008 & .516$\pm$.011 & .549$\pm$.010 & .560$\pm$.016 & .607$\pm$.019 & .654$\pm$.021\\
\hline
nodes: 40.3 & Alg. Dist. & .452$\pm$.036 & .498$\pm$.035 & .524$\pm$.021 & .535$\pm$.027 & .531$\pm$.029 & .590$\pm$.032 & .652$\pm$.044\\
\hline
edges: 96.6 & OTC & {\bf .555$\pm$.007} & {\bf .615$\pm$.003} & {\bf .658$\pm$.006} & {\bf .675$\pm$.010} & {\bf .698$\pm$.003} & {\bf .756$\pm$.006} & {\bf .781$\pm$.004}\\
\hline
\toprule 
{\bf BZR\_MD} & REC & .525$\pm$.011 & .548$\pm$.015 & .563$\pm$.020 & .553$\pm$.021 & .563$\pm$.012 & .569$\pm$.012 & .587$\pm$.020\\
\hline
graphs: 306 & Heavy & .497$\pm$.000 & .546$\pm$.000 & .555$\pm$.000 & .522$\pm$.000 & .550$\pm$.000 & .572$\pm$.000 & .558$\pm$.000\\
\hline
classes: 2 & Affinity & .508$\pm$.006 & .534$\pm$.012 & .534$\pm$.017 & .532$\pm$.015 & .549$\pm$.020 & .567$\pm$.033 & .562$\pm$.029\\
\hline
nodes: 21.3 & Alg. Dist. & .497$\pm$.021 & .546$\pm$.026 & .555$\pm$.038 & .522$\pm$.028 & .550$\pm$.028 & .572$\pm$.024 & .558$\pm$.039\\
\hline
edges: 225.06 & OTC & {\bf .534$\pm$.000} & {\bf .569$\pm$.000} & {\bf .547$\pm$.000} & {\bf .579$\pm$.000} & {\bf .572$\pm$.000} & {\bf .607$\pm$.000} & {\bf .603$\pm$.000}\\
\hline
\toprule 
{\bf Mutagenicity} & REC & .713$\pm$.006 & .730$\pm$.006 & .742$\pm$.005 & .752$\pm$.004 & .758$\pm$.005 & .765$\pm$.007 & .769$\pm$.007\\
\hline
graphs: 4337 & Heavy & .718 $\pm$.006 & .738$\pm$.004 & .753$\pm$.004 & .763$\pm$.004 & .771$\pm$.003 & .779$\pm$.004 & .783$\pm$.004\\
\hline
classes: 2 & Affinity & - & - & - & - & - & - & -\\
\hline
nodes: 30.3 & Alg. Dist. & - & - & - & - & - & - & -\\
\hline
edges: 30.8 & OTC & {\bf .750$\pm$.004} & {\bf .767$\pm$.003} & {\bf .776$\pm$.002} & {\bf .782$\pm$.002} & {\bf .788$\pm$.003} & {\bf .792$\pm$.003} & {\bf .801$\pm$.004}\\
\hline
\toprule 

 \end{tabular} 
  %\end{center} 
  \label{default} 
  \end{table*}

==> table50.tex <==
\begin{table*}[t!]  \caption{{\bf Description of graph datasets, and comparison of accuracy on test data.}  We provide the statistics on the number of graphs, number of classes, average number of nodes, and average number of edges in each dataset. The classification test accuracy (along with standard deviation) when each graph was (roughly) compressed to half is shown for each method for each training fraction in $\{0.2, \ldots, 0.8\}$.  The algorithm having the best performance is indicated with bold in each case. '-' entries indicate that the method failed to compress the given dataset due to a matrix singularity.  
  \label{tab:compare}}   
  \vskip 0.1in 
  \addtolength{\tabcolsep}{-4.5pt} 
 \centering  
 %\begin{center} 
 \small 
  \begin{tabular} {|c|c|c|c|c|c|c|c|c|c|} %{*{12}{c}} %{p{0.32in}d|d|ddddddd} 
  \toprule 
   Dataset &  method &  acc@0.2 &  acc@0.3 & acc@0.4 &  acc@0.5 &  acc@0.6 &  acc@0.7 & acc@0.8 \\   \hline 
  \toprule 
 
{\bf MSRC\_9} & REC & .738$\pm$.011 & .782$\pm$.010 & .817$\pm$.009 & .818$\pm$.013 & .835$\pm$.020 & .833$\pm$.018 & .840$\pm$.013\\
\hline
graphs: 221 & Heavy & .648$\pm$.019 & .710$\pm$.024 & .766$\pm$.014 & .773$\pm$.010 & .786$\pm$.009 & .796$\pm$.010 & .813$\pm$.009\\
\hline
classes: 8 & Affinity & .665$\pm$.015 & .722$\pm$.005 & .762$\pm$.010 & .774$\pm$.014 & .789$\pm$.026 & .786$\pm$.019 & .801$\pm$.017\\
\hline
nodes: 40.6 & Algebraic & .666$\pm$.048 & .717$\pm$.051 & .756$\pm$.029 & .771$\pm$.039 & .798$\pm$.032 & .803$\pm$.030 & .809$\pm$.046\\
\hline
edges: 97.9 & OTC  & {\bf .794$\pm$.004} & {\bf .819$\pm$.003} & {\bf .833$\pm$.005} & {\bf .850$\pm$.002} & {\bf .844$\pm$.007} & {\bf .850$\pm$.001} & {\bf .861$\pm$.008}\\
\hline
\toprule 
{\bf DHFR} & REC & .681$\pm$.011 & .704$\pm$.014 & .724$\pm$.007 & .738$\pm$.009 & .749$\pm$.008 & .756$\pm$.011 & .771$\pm$.011\\
\hline
graphs: 467 & Heavy & .719$\pm$.010 & .751$\pm$.010 & .776$\pm$.012 & .782$\pm$.008 & .777$\pm$.009 & .786$\pm$.014 & .799$\pm$.013\\
\hline
classes: 2 & Affinity & .717$\pm$.013 & .733$\pm$.011 & .745$\pm$.014 & .761$\pm$.014 & .771$\pm$.019 & .767$\pm$.015 & .785$\pm$.013\\
\hline
nodes: 42.4 & Algebraic & .743$\pm$.011 & .761$\pm$.012 & .768$\pm$.022 & .786$\pm$.019 & {\bf .810$\pm$.025} & {\bf .817$\pm$.033} & .809$\pm$.030\\
\hline
edges: 44.5 & OTC & {\bf .755$\pm$.007} & {\bf .781$\pm$.005} & {\bf .787$\pm$.005} & {\bf .793$\pm$.007} &  .805$\pm$.010 &  .810$\pm$.014 & {\bf .818$\pm$.008}\\
\hline
\toprule 
{\bf MSRC\_21C} & REC & .485$\pm$.016 & .543$\pm$.010 & .595$\pm$.010 & .625$\pm$.013 & .641$\pm$.008 & .696$\pm$.013 & .738$\pm$.016\\
\hline
graphs: 209 & Heavy & .408$\pm$.016 & .479$\pm$.015 & .516$\pm$.009 & .538$\pm$.009 & .557$\pm$.011 & .602$\pm$.022 & .653$\pm$.011\\
\hline
classes: 20 & Affinity & .413$\pm$.021 & .489$\pm$.008 & .516$\pm$.011 & .549$\pm$.010 & .560$\pm$.016 & .607$\pm$.019 & .654$\pm$.021\\
\hline
nodes: 40.3 & Algebraic & .452$\pm$.036 & .498$\pm$.035 & .524$\pm$.021 & .535$\pm$.027 & .531$\pm$.029 & .590$\pm$.032 & .652$\pm$.044\\
\hline
edges: 96.6 & OTC & {\bf .550$\pm$.004} & {\bf .612$\pm$.005} & {\bf .648$\pm$.005} & {\bf .674$\pm$.004} & {\bf .697$\pm$.008} & {\bf .751$\pm$.009} & {\bf .777$\pm$.002}\\
\hline
\toprule 
{\bf BZR\_MD} & REC & .525$\pm$.011 & .548$\pm$.015 & {\bf .563$\pm$.020} & .553$\pm$.021 & .563$\pm$.012 & .569$\pm$.012 & .587$\pm$.020\\
\hline
graphs: 306 & Heavy & .497$\pm$.000 & .546$\pm$.000 & .555$\pm$.000 & .522$\pm$.000 & .550$\pm$.000 & .572$\pm$.000 & .558$\pm$.000\\
\hline
classes: 2 & Affinity & .508$\pm$.006 & .534$\pm$.012 & .534$\pm$.017 & .532$\pm$.015 & .549$\pm$.020 & .567$\pm$.033 & .562$\pm$.029\\
\hline
nodes: 21.3 & Algebraic & .497$\pm$.021 & .546$\pm$.026 & .555$\pm$.038 & .522$\pm$.028 & .550$\pm$.028 & .572$\pm$.024 & .558$\pm$.039\\
\hline
edges: 225.1 & OTC & {\bf .534$\pm$.000} & {\bf .569$\pm$.000} &  .547$\pm$.000 & {\bf .579$\pm$.000} & {\bf .572$\pm$.000} & {\bf .607$\pm$.000} & {\bf .603$\pm$.000}\\
\hline
\toprule 
{\bf Mutagenicity} & REC & .713$\pm$.006 & .730$\pm$.006 & .742$\pm$.005 & .752$\pm$.004 & .758$\pm$.005 & .765$\pm$.007 & .769$\pm$.007\\
\hline
graphs: 4337 & Heavy & .718 $\pm$.006 & .738$\pm$.004 & .753$\pm$.004 & .763$\pm$.004 & .771$\pm$.003 & .779$\pm$.004 & .783$\pm$.004\\
\hline
classes: 2 & Affinity & - & - & - & - & - & - & -\\
\hline
nodes: 30.3 & Algebraic & - & - & - & - & - & - & -\\
\hline
edges: 30.8 & OTC & {\bf .750$\pm$.004} & {\bf .767$\pm$.003} & {\bf .776$\pm$.002} & {\bf .782$\pm$.002} & {\bf .788$\pm$.003} & {\bf .792$\pm$.003} & {\bf .801$\pm$.004}\\
\toprule 
 \end{tabular} 
  %\end{center} 
  \label{default} 
  \end{table*}
